Neuronal Correlation: a Central Concept in Neural Network

This paper proposes to study neural networks through neuronal correlation, a statistical measure of correlated neuronal activity on the penultimate layer. We show that neuronal correlation can be efficiently estimated via weight matrix, can be effectively enforced through layer structure, and is a strong indicator of generalisation ability of the network. More importantly, we show that neuronal correlation significantly impacts on the accuracy of entropy estimation in high-dimensional hidden spaces. While previous estimation methods may be subject to significant inaccuracy due to implicit assumption on neuronal independence, we present a novel computational method to have an efficient and authentic computation of entropy, by taking into consideration the neuronal correlation. In doing so, we install neuronal correlation as a central concept of neural network.

==> reply.tex <==
Thanks to the reviewers for providing comments timely at this difficult time. We are very grateful that all three reviewers recognise the novelty and originality of the paper.  We have tried our best to explain all the aspects of our main view -- neuronal correlation could be a key concept of DNN theoretical study -- as given in Figure 1; however, we are limited by the pages and the number of aspects that we believe are needed to support our view. 
 
In general, we found that, the reviewers’ comments either have already been addressed in the paper, require additional clarification, or can be taken into consideration without affecting the results of the paper. That is, no major issue has been raised. Please find below our detailed response to the reviewers separately. 

Reviewer 1.

Thank you for the comment ``The result on NC is a great first step towards understanding neural networks.'' 

The structure-correlation coefficient expresses the complexity of interactions between neurons on the same layer. The interactions are made indirectly via neurons in the previous layer. As shown in our experiment, higher interaction complexity leads to lower average WC. 

Sections 4.1&4.2 are to show that, after the consideration of NC/WC, our proposed method of computing EN can achieve more accurate result, which in turn can be helpful for understanding GE. 

We respectfully disagree with the comment that our EN estimation by kernel embedding is well known. As far as we know, this is the first time the kernel embedding is introduced for EN estimation, based on our observation -- supported with experiments -- that a direct application of EN estimators on DNNs can bring significant inaccuracy due to loss of information. 

The fact that N6&N7 are trained on CIFAR10 has been mentioned at the beginning of Section 4.  

Reviewer 3:

Thank you for recognising the novelty of our NC and that our experiments answer important questions. 

We first address the comments in Questions, and then clarify the comments in Weaknesses. 

We use cross entropy error function and 0.001 learning rate.

The connection between EN and GE has been widely studied in the literature (eg Tishby et al 2017). This paper does not participate in this discussion, but instead uses a dashed line to show that the existing discussion has not settled a theoretical relation between them. 

We follow a common practice to study the penultimate layer. Nevertheless, our approach can be applied to other layers. 

For the weaknesses: 

While there may be minor difference over "GE over loss" and "GE over error", we are very confident that our results can be extended to GE over error. The loss at the penultimate layer and the error at the output layer are positively correlated over a fixed, deterministic Softmax function. Our methods are not affected by any fixed, deterministic function. 

We actually conducted experiments on many more networks with different hyper-parameters. All experiments show similar results, and for this reason, we only report results on a few typical networks -- others do not give more information. 

We are mainly concerning the trend of GE, instead of the GE value itself, as shown in our experiments. So, it is unclear how the early stopping can play a role here. Actually, we can study any snapshot in our experiment (Figure 7) but believe that does not change our results. 

We will extend our curves to include the first few epochs. 


Reviewer 4: 

Thank you for recognising the originality of the paper and that the kernel embedding for entropy estimation is a good solution. 

Below, we first answer questions in Comments and then address those in Improvements. 

The constraint is low training error. 

We do not omit Sigma_{l-1}. Instead, we notice that (1) it remains stable across epochs and (2) it can be iteratively computed until reaching the input layer. 

The guideline is that, to have a lower WC, we need to design a layer which has larger structural correlation coefficient. While this is a heuristic result as indicated in the paper, it works for all networks in our experiments, including convolutional networks for CIFAR10. 

The error range is the range to include all possible values across layers. Since theoretically the values should be the same across layers, the difference of the ranges between two methods exhibits the accuracy improvement of our method. 

Below, due to space limit, we answer questions 4-6 in the Improvement, and can assure the reviewer that questions 1-3 can either be addressed or have already been addressed (we cannot get the experiment data in the department due to the lockdown for COVID-19). 

There are two factors affecting the precision of the EN computation: kernel parameters and the numerical error. As far as we observe from experiments, the former has more weights on the final result. But thank you for the suggestion: a controlled experiment will be helpful. 

We have shown in experiments (Sections 4.1&4.2) that high-order correlation significantly affects the EN computation. With kernel embedding, the precision of EN computation has theoretical guarantee. 

Existing methods cannot be easily adapted. Section 4.1 is the experiment to show the difference with and without kernel embedding. 
